Language Agent Tree Search Unifies Reasoning Acting and Planning in Language Models

While language models (LMs) have shown potential across a range of decision-making tasks, their reliance on simple acting processes limits their broad deployment as autonomous agents. In this paper, we introduce Language Agent Tree Search (LATS) -- the first general framework that synergizes the capabilities of LMs in reasoning, acting, and planning. By leveraging the in-context learning ability of LMs, we integrate Monte Carlo Tree Search into LATS to enable LMs as agents, along with LM-powered value functions and self-reflections for proficient exploration and enhanced decision-making. A key feature of our approach is the incorporation of an environment for external feedback, which offers a more deliberate and adaptive problem-solving mechanism that surpasses the constraints of existing techniques. Our experimental evaluation across diverse domains, including programming, interactive question-answering (QA), web navigation, and math, validates the effectiveness and generality of LATS in decision-making while maintaining competitive or improved reasoning performance. Notably, LATS achieves state-of-the-art pass@1 accuracy (92.7%) for programming on HumanEval with GPT-4 and demonstrates gradient-free performance (average score of 75.9) comparable to gradient-based fine-tuning for web navigation on WebShop with GPT-3.5. Code can be found at https://github.com/lapisrocks/LanguageAgentTreeSearch

==> tables/comparison.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lc}
\toprule
\textbf{Prompt Method} & \textbf{HotpotQA (EM)} \\
\midrule
LATS (w=0.5) & 0.55 \\
LATS (w=2.0) & 0.61 \\
LATS (d=4) & 0.58 \\
LATS (CoT) & 0.60 \\
LATS (No LM Heuristic) & 0.37  \\
LATS & 0.61 \\
\bottomrule
\end{tabular}
\caption{Ablation results on LATS and baseline variants in HotPotQA. LATS requires every component and operation for optimal performance.}
\label{tab:lats_ablations}
\end{table}

